On the Computational Complexity of Generalized Common Shape Puzzles

In this study, we investigate the computational complexity of some variants of generalized puzzles. We are provided with two sets S_1 and S_2 of polyominoes. The first puzzle asks us to form the same shape using polyominoes in S_1 and S_2. We demonstrate that this is polynomial-time solvable if S_1 and S_2 have constant numbers of polyominoes, and it is strongly NP-complete in general. The second puzzle allows us to make copies of the pieces in S_1 and S_2. That is, a polyomino in S_1 can be used multiple times to form a shape. This is a generalized version of the classical puzzle known as the common multiple shape puzzle. For two polyominoes P and Q, the common multiple shape is a shape that can be formed by many copies of P and many copies of Q. We show that the second puzzle is undecidable in general. The undecidability is demonstrated by a reduction from a new type of undecidable puzzle based on tiling. Nevertheless, certain concrete instances of the common multiple shape can be solved in a practical time. We present a method for determining the common multiple shape for provided tuples of polyominoes and outline concrete results, which improve on the previously known results in puzzle society.

==> app-const.tex <==

The complete reduction from a given instance $s_1=(b;ca),s_2=(a;ab),s_3=(ca;a),s_4=(abc;c)$
of the Post correspondence problem to the jigsaw puzzle is depicted in \figurename~\ref{fig:post-sample-c}.

\begin{figure}[thb]\centering
\includegraphics[bb=0 0 345 604,width=0.8\textwidth]{./figure/post-sample-c.pdf}
\caption{Construction of a solution of the jigsaw puzzle from a solution of the instance of the Post corresponding problem}
\label{fig:post-sample-c}
\end{figure} 


==> figure/shape-logic.tex <==

In this section, we focus on the generalized shape logic puzzle.
That is, we are given two sets $\calS_1$ and $\calS_2$ of polyominoes, and 
we have to decide if all pieces in $\calS_1$ (and in $\calS_2$) can form some polyomino $X$ in common.

\begin{obs}
\label{obs:poly}
When $\msize{\calS_1}+\msize{\calS_2}$ is a constant $k$, 
the generalized shape logic puzzle can be solved in polynomial time of $n$, 
where $n$ is the total number of vertices in $\calS_1\cup\calS_2$.
\end{obs}
\begin{proof}(Outline.)
We solve the problem by brute force, 
and we use the same proof technique in \cite[Section 3]{DKKMORRUU2020}.
In \cite[Section 3]{DKKMORRUU2020}, the authors give the way to solve the symmetric assembly puzzle,
that asks to form a symmetric shape by using the pieces in a set of (general) simple polygons, in a polynomial time.

We can reduce the generalized shape logic puzzle to the symmetric shape puzzle in a polynomial time as follows.
We suppose that the generalized shape logic puzzle has a solution and 
the pieces in $\calS_1$ forms a polygon $P$, which also can be formed by the pieces in $\calS_2$.
Then, without loss of generality, $P$ can be put so that $P$ has the rightmost vertex $v$ on $\partial P$.
that is, any point in $P$ is not right of $v$.
Now joining $P$ and its mirror image $P^R$ at the vertex $v$ with its mirror image on $\partial P^R$,
we obtain a symmetric shape.
That is, when the shape logic puzzle with $\calS_1$ and $\calS_2$ has a solution,
the symmetric shape puzzle also has a solution for $\calS_1\cup\calS_2$ such that the left half of the symmetric shape consists of 
the pieces in $\calS_1$, and the right half of the symmetric shape consists of the pieces in $\calS_2$.
Here the proof in \cite[Section 3]{DKKMORRUU2020} is based on a brute force.
Therefore, we can restrict ourselves to search a symmetric shape that also gives us a solution for the shape logic puzzle on $\calS_1\cup\calS_2$.
Since the original brute force algorithm for the symmetric shape puzzle runs in a polynomial time of $n$, 
so does our algorithm.
\qed\end{proof}

\begin{theorem}
The shape logic puzzle is strongly NP-complete even if all pieces in $\calS_1$ and $\calS_2$ are small rectangles.
\end{theorem}

\begin{proof}
By the definition of a small polyomino, the problem is in NP.
Thus we show the NP-hardness by a reduction from the 3-partition problem.
In the 3-partition problem, we are given a multiset of 
$3m$ positive integers $A=\{a_1,a_2,\ldots,a_{3m}\}$, where the $a_i$s are bounded 
above by a polynomial of $m$. 
The goal is to partition the multiset $A$ into $m$ triples such that every triple
has the same sum $B=(\sum_{i=1}^{3m}a_i)/m$.
It is known that the 3-partition problem is strongly NP-complete even if every $a_i$ satisfies $B/4<a_i<B/2$  \cite[SP16]{GJ79}.
Without loss of generality, we assume that $a_i>3$ for each $i$ and $B=3mB'$ for some positive integer $B'$.
%and $m=2m'$ for some positive integers $B'$ and $m'$.

Then the set $\calS_1$ consists of $3m$ rectangles of size $1\times (a_i+3m^2)$ for each $i=1,2,\ldots,3m$.
On the other hand, $\calS_2$ consists of $3m$ congruent rectangles of size $m\times (B/(3m)+3m)$.
The construction can be done in a polynomial time of $m$.

We then can observe that $3m<B/(3m)+3m<B/4+3m^2<a_i+3m^2$ for each $i$ since we have $3m$ pieces in $\calS_1$, $a_i>3$, and $a_i>B/4$.
That is, (1) $B/(3m)+3m$ is larger than $3m$, which is the number of sticky rectangles in $\calS_1$, and
(2) each $a_i+3m^2$ cannot fit into any rectangle formed by pieces in $\calS_2$ except we make a rectangle of width $m$.
Therefore, to form the same shape by the pieces in $\calS_1$ and the pieces in $\calS_2$,
the only way is forming the rectangle of size $m\times(B+9m^2)$ by the pieces in $\calS_2$,
and packing the long rectangles of size $1\times (a_i+3m^2)$ into this frame.
The arrangement of pieces in $\calS_1$ directly gives us the solution of the original instance of the 3-partition problem.
\qed\end{proof}





==> patterns.tex <==

In this section, in addition to the patterns in Section \ref{sec:implementation},
we provide more new patterns which improve previously known patterns.
The notation for small polyominoes follows ones given in the following wab pages.
(They are rather trivial as you can see in the patterns.)
%Similarly, 

